S2SD: Simultaneous Similarity-based Self-Distillation for Deep Metric Learning

Deep Metric Learning (DML) provides a crucial tool for visual similarity and zero-shot applications by learning generalizing embedding spaces, although recent work in DML has shown strong performance saturation across training objectives. However, generalization capacity is known to scale with the embedding space dimensionality. Unfortunately, high dimensional embeddings also create higher retrieval cost for downstream applications. To remedy this, we propose \emph{Simultaneous Similarity-based Self-distillation (S2SD). S2SD extends DML with knowledge distillation from auxiliary, high-dimensional embedding and feature spaces to leverage complementary context during training while retaining test-time cost and with negligible changes to the training time. Experiments and ablations across different objectives and standard benchmarks show S2SD offers notable improvements of up to 7% in Recall@1, while also setting a new state-of-the-art. Code available at https://github.com/MLforHealth/S2SD.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

==> tables/Short_Full_Results_arxiv.tex <==
\begin{table}[t]
    \caption{\textit{S2SD comparison against strong baseline objectives.} All results computed over multiple seeds. \textbf{Bold} denotes best results per loss \& benchmark,  \blue{\textbf{bluebold}} marks best results per benchmark.}
 \footnotesize
   \setlength\tabcolsep{1.4pt}
   \centering
   %\begin{tabular}{l|c|ccc|c}
   \resizebox{\textwidth}{!}{
   \begin{tabular}{l|c|c||c|c||c|c}
     \toprule
     \multicolumn{1}{l}{\textbf{Benchmark}$\rightarrow$} & \multicolumn{2}{c}{\textsc{CUB200-2011}} & \multicolumn{2}{c}{\textsc{CARS196}} & \multicolumn{2}{c}{\textsc{SOP}} \\
     \midrule
     \textbf{Approaches} $\downarrow$ & R@1 & NMI & R@1 & NMI & R@1 & NMI\\
    \midrule
    \textbf{Margin}, $\beta=1.2$, \citep{margin} & $63.09\pm0.46$ & $68.21\pm0.33$ & $79.86\pm0.33$ & $67.36\pm0.34$ & $78.43\pm0.07$ & $90.40\pm0.03$\\        
    + DSD & $65.11\pm0.18$ & $69.65\pm0.44$ & $83.19\pm0.18$ & $69.28\pm0.56$ & $79.05\pm0.12$ & $90.52\pm0.18$\\
    + MSD & $66.13\pm0.34$ & $70.83\pm0.27$ & $83.63\pm0.31$ & $69.80\pm0.36$ & $79.26\pm0.15$ & $90.60\pm0.10$\\
    + MSDF & $\mathbf{67.58\pm0.32}$ & $\mathbf{71.47\pm0.19}$ & $85.55\pm0.23$ & $\mathbf{71.68\pm0.54}$ & \blue{$\mathbf{79.63\pm0.15}$} & \blue{$\mathbf{90.70\pm0.09}$} \\
    + MSDFA & $67.21\pm0.23$ & $71.43\pm0.25$ & $\mathbf{86.45\pm0.35}$ & $71.46\pm0.24$ & $78.82\pm0.09$ & $90.49\pm0.06$ \\
    \hline
    \textbf{R-Margin}, $\beta=0.6$, \citep{roth2020revisiting} & $64.93\pm0.42$ & $68.36\pm0.32$ & $82.37\pm0.13$ & $68.66\pm0.47$ & $77.58\pm0.11$ & $90.42\pm0.03$\\ 
    + DSD & $66.58\pm0.08$ & $70.03\pm0.41$ & $84.64\pm0.16$ & $70.87\pm0.18$ & $77.86\pm0.10$ & $90.50\pm0.03$\\
    + MSD & $66.81\pm0.27$ & $70.47\pm0.16$ & $85.01\pm0.10$ & $71.67\pm0.40$ & $78.00\pm0.06$ & $90.47\pm0.04$\\
    + MSDF & $68.12\pm0.30$ & $\mathbf{71.80\pm0.33}$ & $85.78\pm0.22$ & $\mathbf{72.24\pm0.31}$ & $\mathbf{78.57\pm0.09}$ & $\mathbf{90.58\pm0.02}$\\
    + MSDFA & $\blue{\mathbf{68.58\pm0.26}}$ & $71.64\pm0.40$ & $\blue{\mathbf{86.81\pm0.35}}$ & $71.48\pm0.29$ & $78.00\pm0.11$ & $90.41\pm0.02$\\
    \hline
    \textbf{Multisimilarity} \citep{multisimilarity} & $62.80\pm0.70$ & $68.55\pm0.38$ & $81.68\pm0.19$ & $69.43\pm0.38$ & $77.99\pm0.09$ & $90.00\pm0.02$\\
    + DSD & $65.57\pm0.26$ & $70.08\pm0.33$ & $83.51\pm0.20$ & $70.30\pm0.05$ & $78.23\pm0.04$ & $90.08\pm0.04$\\
    + MSD & $65.80\pm0.16$ & $70.6553\pm0.01$ & $83.98\pm0.10$ & $71.34\pm0.09$ & $78.42\pm0.09$ & $90.09\pm0.03$\\        
    + MSDF & $67.04\pm0.29$ & $\blue{\mathbf{71.87\pm0.19}}$ & $85.69\pm0.19$ & $\blue{\mathbf{72.77\pm0.13}}$ & $\mathbf{78.59\pm0.08}$ & $\mathbf{90.09\pm0.06}$\\
    + MSDFA & $\mathbf{67.68\pm0.29}$ & $71.40\pm0.21$ & $\mathbf{85.89\pm0.15}$ & $71.45\pm0.26$ & $78.07\pm0.06$ & $89.88\pm0.10$ \\
         
    % \hline
    % \textbf{ProxyAnchor} \citep{kim2020proxy} & $64.58\pm0.23$ & $68.95\pm0.24$ & $82.55\pm0.41$ & $69.49\pm0.30$ & $77.92\pm0.09$ & $90.09\pm0.06$\\    
    % + DSD    & $65.50\pm0.47$ & $69.97\pm0.55$ & $83.52\pm0.11$ & $70.76\pm0.17$ & $78.33\pm0.08$ & $90.24\pm0.06$\\
    % + MSDF & $\mathbf{66.71\pm0.12}$ & $70.60\pm0.24$ & $85.20\pm0.09$ & $\mathbf{71.19\pm0.18}$ & $\mathbf{78.50\pm0.04}$ & $\mathbf{90.31\pm0.03}$\\
    % + MSDFA & $66.47\pm0.36$ & $\mathbf{70.66\pm0.17}$ & $\mathbf{85.59\pm0.17}$ & $69.77\pm0.45$ & $78.03\pm0.05$ & $90.18\pm0.03$\\
    \bottomrule
    \end{tabular}}
    \label{tab:relative_results}
    % \vspace{-13pt}
 \end{table}


% \begin{table*}[t]
%  \small
%  \rowcolors{2}{gray!8}{white}
%   \setlength\tabcolsep{1.4pt}
%   \centering
%   %\begin{tabular}{l|c|ccc|c}
%   \begin{tabular}{l|c|c||c|c||c|c}
%      \toprule
%      \multicolumn{1}{l}{Benchmarks$\rightarrow$} & \multicolumn{2}{c}{CUB200-2011} & \multicolumn{2}{c}{CARS196} & \multicolumn{2}{c}{SOP} \\
%      \midrule
%      Approaches $\downarrow$ & R@1 & NMI & R@1 & NMI & R@1 & NMI\\
%      \midrule
%     Imagenet~\cite{imagenet} & $43.77$ & $57.56$ & $36.39$ & $37.96$ & $48.65$ & $58.64$ \\
%     \midrule
%     Angular~\cite{angular} & $62.10\pm0.27$ & $67.59\pm0.26$ & $78.00\pm0.32$ & $66.48\pm0.44$ & $73.22\pm0.07$ & $89.53\pm0.01$\\
%     ArcFace~\cite{arcface} & $62.67\pm0.67$ & $67.66\pm0.38$ & $79.16\pm0.97$ & $66.99\pm1.08$ & $77.71\pm0.15$ & $90.09\pm0.03$\\
%     Contrastive~\cite{contrastive} (D) & $61.50\pm0.17$ & $66.45\pm0.27$ & $75.78\pm0.39$ & $64.04\pm0.13$ & $73.21\pm0.04$ & $89.78\pm0.02$\\
%     Margin (D, $\beta=0.6$)~\cite{margin} & $62.50\pm0.24$ & $67.02\pm0.37$ & $77.70\pm0.32$ & $65.29\pm0.32$ & $77.38\pm0.11$ & \blue{$\mathbf{90.45\pm0.03}$}\\
%     Margin (D, $\beta=1.2$)~\cite{margin} & $\mathbf{63.09\pm0.46}$ & $68.21\pm0.33$ & $79.86\pm0.33$ & $67.36\pm0.34$ & $\mathbf{78.43\pm0.07}$ & $90.40\pm0.03$\\
%     Multisimilarity~\cite{multisimilarity} & $62.80\pm0.70$ & \blue{$\mathbf{68.55\pm0.38}$} & $\mathbf{81.68\pm0.19}$ & \blue{$\mathbf{69.43\pm0.38}$} & $77.99\pm0.09$ & $90.00\pm0.02$\\
%     Npair~\cite{npairs} & $61.63\pm0.58$ & $67.64\pm0.37$ & $77.48\pm0.28$ & $66.55\pm0.19$ & $75.86\pm0.08$ & $89.79\pm0.03$\\
%     Pnca~\cite{proxynca} & $62.80\pm0.48$ & $66.93\pm0.38$ & $78.48\pm0.58$ & $65.76\pm0.22$ & $-$ & $-$\\
%     SNR (D)~\cite{signal2noise} & $62.88\pm0.18$ & $67.16\pm0.25$ & $78.69\pm0.19$ & $65.84\pm0.52$ & $77.61\pm0.34$ & $90.10\pm0.08$\\
%     Softmax~\cite{zhai2018classification} & $61.66\pm0.33$ & $66.77\pm0.36$ & $78.91\pm0.27$ & $66.35\pm0.30$ & $76.92\pm0.64$ & $89.82\pm0.15$\\
%     \midrule
%     Triplet (D)~\cite{margin} & $62.87\pm0.35$ & $67.53\pm0.14$ & $79.13\pm0.27$ & $65.90\pm0.18$ & $77.39\pm0.15$ & $90.06\pm0.02$\\
%     Triplet (R)~\cite{semihard} & $58.48\pm0.31$ & $63.84\pm0.30$ & $70.63\pm0.43$ & $61.09\pm0.27$ & $67.86\pm0.14$ & $88.35\pm0.04$\\
%     \midrule
%     R-Margin (D, $\beta=0.6$) & \blue{$\mathbf{64.93\pm0.42}$} & $68.36\pm0.32$ & \blue{$\mathbf{82.37\pm0.13}$} & $68.66\pm0.47$ & $77.58\pm0.11$ & $90.42\pm0.03$\\

%     \bottomrule
%     \end{tabular}
%     \caption{\textit{Comparison of Recall@1 and NMI performances against various objectives} averaged over 5 runs.}
%     \label{tab:relative_results}
% \vspace{-8pt}
%  \end{table*}


==> tables/old_sota.tex <==
\begin{table*}[t]
    \caption{\textit{State-of-the-art comparison.} We show that our self-distillation module (\textit{SMSD}) achieves state-of-the-art across literature. ($^*$) stands for IBN with frozen Batch-Norm, ($^\dagger$) notes global max- \& average pooling throughout \citep{kim2020proxy}. ($^+$) means larger images used.}
    \setlength\tabcolsep{1.5pt}
    \footnotesize
    \centering
    \resizebox{\textwidth}{!}{
     \begin{tabular}{l||c|c|c||c|c|c||c|c|c}
         \toprule
         Benchmark $\rightarrow$ & \multicolumn{3}{c}{CUB200-2011} & \multicolumn{3}{c}{CARS196}& \multicolumn{3}{c}{SOP}\\
         \midrule
         Approach $\downarrow$ & R@1 & R@2 & NMI & R@1 & R@2 & NMI & R@1 & R@10 & NMI \\
         \midrule
         \hline
         \multicolumn{10}{>{\columncolor[gray]{.8}}l}{\textbf{ResNet50-128}} \\
         \hline
         \rowcolor{vvlightgray}
         D\&C \citep{Sanakoyeu_2019_CVPR}  & 65.9 & 76.6 & 69.6 & 84.6 & 90.7 & 70.3 & 75.9 & 88.4 & 90.2\\
         \rowcolor{vvlightgray}
         MIC \citep{mic}                   & 66.1 & 76.8 & 69.7 & 82.6 & 89.1 & 68.4 & 77.2 & 89.4 & 90.0\\
         \rowcolor{vvlightgray}
         PADS \citep{roth2020pads}         & 67.3 & 78.0 & 69.9 & 83.5 & 89.7 & 68.8 & 76.5 & 89.0 & 89.9\\
         \hline
         Multisimilarity+\textit{SMSD}     & 68.0  $\pm$  0.2 & 78.7 $\pm$ 0.1 & 71.7 $\pm$ 0.4 & 86.3 $\pm$ 0.1 & 91.8 $\pm$ 0.3 & 72.0 $\pm$ 0.3 & 79.0 $\pm$ 0.2 & 90.2 $\pm$ 0.1 & 90.6 $\pm$ 0.1\\
         Margin+\textit{SMSD}            & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & 80.2 $\pm$ 0.2 & 91.5 $\pm$ 0.1 & 90.9 $\pm$ 0.1\\
         R-Margin+\textit{SMSD}          & \textbf{68.9}  $\pm$  \textbf{0.3} & \textbf{79.0} $\pm$ \textbf{0.3} & \textbf{72.1} $\pm$ \textbf{0.4} & \textbf{87.6} $\pm$ \textbf{0.2} & \textbf{92.7} $\pm$ \textbf{0.2} & \textbf{72.3} $\pm$ \textbf{0.2} & 79.2 $\pm$ 0.2 & 90.3 $\pm$ 0.1 & 90.8 $\pm$ 0.1\\
         \midrule
         \hline
         \multicolumn{10}{>{\columncolor[gray]{.8}}l}{\textbf{ResNet50-512}} \\
         \hline
         \rowcolor{vvlightgray}
         DiVA \citep{milbich2020diva}   & 69.2 & 79.3 & 71.4 & 87.6 & 92.9 & 72.2 & 79.6 & 91.2 & 90.6\\
         \hline
         Multisimilarity+\textit{SMSD}  & 69.2 $\pm$ 0.1 & 79.1 $\pm$ 0.2 & 71.4 $\pm$ 0.2 & 89.1 $\pm$ 0.2 & 93.8 $\pm$ 0.2 & 74.0 $\pm$ 0.2 & - & - & -\\
         Margin+\textit{SMSD}           & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ -\\
         R-Margin+\textit{SMSD}         & 69.7 $\pm$ 0.2 & 79.5 $\pm$ 0.3 & 71.6 $\pm$ 0.2 & 89.5 $\pm$ 0.2 & 93.8 $\pm$ 0.3 & 72.9 $\pm$ 0.3 & - $\pm$ - & - $\pm$ - & - $\pm$ -\\
         % \red{N} DiVA+\textit{SMSD}     & - & - & - & - & - & - & - & - & -\\
         \midrule
         \hline
         \multicolumn{10}{>{\columncolor[gray]{.8}}l}{\textbf{Inception-BN-512}} \\
         \hline
         \rowcolor{vvlightgray}
         HORDE$^+$ \citep{horde}         & 66.3 & 76.7 & -      & 83.9 & 90.3 & -      & 80.1      & 91.3      & -     \\
         \rowcolor{vvlightgray}
         DiVA \citep{milbich2020diva}    & 66.8 & 77.7 & 70.0 & 84.1 & 90.7 & 68.7 & 78.1 & 90.6 & 90.4\\
         \hline
         Multisimilarity+\textit{SMSD}   & 66.6 $\pm$ 0.3 & 77.5 $\pm$ 0.3 & 70.5 $\pm$ 0.2 & 83.6 $\pm$ 0.3 & 90.3 $\pm$ 0.2 & 69.8 $\pm$ 0.3 & 78.5 $\pm$ 0.2 & 90.6 $\pm$ 0.2 & 90.6 $\pm$ 0.1\\
         Margin+\textit{SMSD}            & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ -\\
         R-Margin+\textit{SMSD}          & 67.4 $\pm$ 0.3 & 78.0 $\pm$ 0.4 & 70.3 $\pm$ 0.2 & 83.8 $\pm$ 0.3 & 90.3 $\pm$ 0.2 & 69.4 $\pm$ 0.2 & - & - & -\\
         \hline
         \rowcolor{vvlightgray}
         Softtriple$^*$ \citep{softriple}              & 65.4 & 76.4 & -      & 84.5 & 90.7 & 70.1 & 78.3 & 90.3 & 92.0\\
         \rowcolor{vvlightgray}
         Multisimilarity$^*$ \citep{multisimilarity}   & 65.7 & 77.0 & -      & 84.1 & 90.4 & -      & 78.2 & 90.5 & -     \\
         \hline
         Multisimilarity$^*$+\textit{SMSD}             & 68.2 $\pm$ 0.3 & 79.1 $\pm$ 0.2 & 71.6 $\pm$ 0.2 & 86.3 $\pm$ 0.2 & 92.2 $\pm$ 0.2 & 72.0 $\pm$ 0.3 & 78.9 $\pm$ 0.2 & - $\pm$ - & 90.6 $\pm$ 0.1\\
         Margin$^*$+\textit{SMSD}                      & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ -\\
         R-Margin$^*$+\textit{SMSD}                    & 69.6 $\pm$ 0.3 & 79.7 $\pm$ 0.3 & 71.2 $\pm$ 0.1 & 86.6 $\pm$ 0.3 & 92.1 $\pm$ 0.3 & 70.9 $\pm$ 0.2 & - & - & -\\
         \hline
         \rowcolor{vvlightgray}
         ProxyAnchor$^{*\dagger}$ \citep{kim2020proxy}   & 68.4  & 79.2       & -            & 86.1 & 91.7 & -    & 79.1 & 90.8 & -\\
         \hline
         Multisimilarity$^{*\dagger}$+\textit{SMSD}      & 69.0 $\pm$ 0.2 & 79.5 $\pm$ 0.2 & 71.7 $\pm$ 0.2 & 87.8 $\pm$ 0.2 & 93.1 $\pm$ 0.2 & 73.3 $\pm$ 0.3 & & &\\
         Margin$^{*\dagger}$+\textit{SMSD}               & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ - & - $\pm$ -\\
         ProxyAnchor$^{*\dagger}$+\textit{SMSD}          & 69.5 $\pm$ 0.2 & 79.8 $\pm$ 0.2 & 71.3 $\pm$ 0.2 & 87.2 $\pm$ 0.3 & 92.6 $\pm$ 0.2 & 70.5 $\pm$ 0.4 & - & - & -\\
         % DiVA+\textit{SMSD}                & 70.1 $\pm$ 0.2 & 80.1 $\pm$ 0.2 & 72.5 $\pm$ 0.3 & - & - & - & - & - & -\\
         \bottomrule
    \end{tabular}}
    \vspace{-5pt}
    \label{tab:sota}
\end{table*}


==> tables/slighly_old_sota.tex <==



\begin{table*}[t]
    \caption{\textit{State-of-the-art comparison.} We show that our self-distillation module (\textit{SMSD}) achieves state-of-the-art across literature. ($^*$) stands for IBN with frozen Batch-Norm, ($^\dagger$) notes global max- \& average pooling throughout \citep{kim2020proxy}.}% ($^+$) means larger images used.}
    \setlength\tabcolsep{1.5pt}
    \footnotesize
    \centering

\resizebox{\textwidth}{!}{
 
 \begin{tabular}{l||c|c|c}
     \toprule
     Benchmark $\rightarrow$ & \multicolumn{3}{c}{CUB200 \citep{cub200-2011}}\\
     \midrule
     Approach $\downarrow$ & R@1 & R@2 & NMI\\
     \midrule
     \hline
     \multicolumn{4}{>{\columncolor[gray]{.8}}l}{\textbf{ResNet50-128}} \\
     \hline
     \rowcolor{vvlightgray}
     Div\&Conq \citep{Sanakoyeu_2019_CVPR}  & 65.9 & 76.6 & 69.6\\
     \rowcolor{vvlightgray}
     MIC \citep{mic}                   & 66.1 & 76.8 & 69.7\\
     \rowcolor{vvlightgray}
     PADS \citep{roth2020pads}         & 67.3 & 78.0 & 69.9\\
     \hline
     Multisimilarity+\textit{SMSD}     & 68.0  $\pm$  0.2 & 78.7 $\pm$ 0.1 & 71.7 $\pm$ 0.4 \\
     Margin+\textit{SMSD}      & 67.6  $\pm$  0.3 & 78.2 $\pm$ 0.2 & 70.8 $\pm$ 0.3 \\
     R-Margin+\textit{SMSD}    & \textbf{68.9}  $\pm$  \textbf{0.3} & \textbf{79.0} $\pm$ \textbf{0.3} & \textbf{72.1} $\pm$ \textbf{0.4} \\
     \midrule
     \hline
     \multicolumn{4}{>{\columncolor[gray]{.8}}l}{\textbf{ResNet50-512}} \\
     \hline
     \rowcolor{vvlightgray}
     EPSHN \citep{epshn}                     & 64.9 & 75.3 &  -   \\
     \rowcolor{vvlightgray}
     NormSoft \citep{zhai2018classification} & 61.3 & 73.9 &  -   \\
     \rowcolor{vvlightgray}
     DiVA \citep{milbich2020diva}            & 69.2 & 79.3 & 71.4 \\
     \hline
     Multisimilarity+\textit{SMSD}  & 69.2 $\pm$ 0.1 & 79.1 $\pm$ 0.2 & 71.4 $\pm$ 0.2 \\
     Margin+\textit{SMSD}           & - $\pm$ - & - $\pm$ - & - $\pm$ -\\
     R-Margin+\textit{SMSD}         & 69.7 $\pm$ 0.2 & 79.5 $\pm$ 0.3 & 71.6 $\pm$ 0.2 \\
     % \red{N} DiVA+\textit{SMSD}     & - & - & - \\
     \midrule
     \hline
     \multicolumn{4}{>{\columncolor[gray]{.8}}l}{\textbf{Inception-BN-512}} \\
     \hline
    %  \rowcolor{vvlightgray}
    %  HORDE$^+$          & 66.3 & 76.7 & - \\
     \rowcolor{vvlightgray}
     DiVA \citep{milbich2020diva}    & 66.8 & 77.7 & 70.0 \\
     \hline
     Multisimilarity+\textit{SMSD}   & 66.6 $\pm$ 0.3 & 77.5 $\pm$ 0.3 & 70.5 $\pm$ 0.2 \\
     Margin+\textit{SMSD}            & 66.8 $\pm$ 0.2 & 77.9 $\pm$ 0.2 & 69.9 $\pm$ 0.3 \\
     R-Margin+\textit{SMSD}          & 67.4 $\pm$ 0.3 & 78.0 $\pm$ 0.4 & 70.3 $\pm$ 0.2 \\
     \hline
     \rowcolor{vvlightgray}
     Softtriple$^*$ \citep{softriple} & 65.4 & 76.4 & -  \\
     \rowcolor{vvlightgray}
     Multisimilarity$^*$ \citep{multisimilarity} & 65.7 & 77.0 & -  \\
     \hline
     Multisimilarity$^*$+\textit{SMSD}             & 68.2 $\pm$ 0.3 & 79.1 $\pm$ 0.2 & 71.6 $\pm$ 0.2 \\
     Margin$^*$+\textit{SMSD}                      & 68.3 $\pm$ 0.2 & 78.8 $\pm$ 0.2 & 71.2 $\pm$ 0.2 \\
     R-Margin$^*$+\textit{SMSD}                    & 69.6 $\pm$ 0.3 & 79.7 $\pm$ 0.3 & 71.2 $\pm$ 0.1 \\
     \hline
     \rowcolor{vvlightgray}
     ProxyAnchor$^{*\dagger}$ \citep{kim2020proxy} & 68.4  & 79.2       & -           \\
     \hline
     Multisimilarity$^{*\dagger}$+\textit{SMSD}      & 69.0 $\pm$ 0.2 & 79.5 $\pm$ 0.2 & 71.7 $\pm$ 0.2 \\
     Margin$^{*\dagger}$+\textit{SMSD}               & 68.3 $\pm$ 0.3 & 78.4 $\pm$ 0.3 & 70.4 $\pm$ 0.2 \\
     ProxyAnchor$^{*\dagger}$+\textit{SMSD}          & 69.5 $\pm$ 0.2 & 79.8 $\pm$ 0.2 & 71.3 $\pm$ 0.2 \\
     % DiVA+\textit{SMSD}                & 70.1 $\pm$ 0.2 & 80.1 $\pm$ 0.2 & 72.5 $\pm$ 0.3 \\
     \bottomrule
\end{tabular}

 \begin{tabular}{l||c|c|c}
     \toprule
     Benchmark $\rightarrow$ & \multicolumn{3}{c}{CARS196 \citep{cars196}}\\
     \midrule
     Approach $\downarrow$ & R@1 & R@2 & NMI \\
     \midrule
     \hline
     \multicolumn{4}{>{\columncolor[gray]{.8}}l}{\textbf{ResNet50-128}} \\
     \hline
     \rowcolor{vvlightgray}
     Div\&Conq \citep{Sanakoyeu_2019_CVPR} & 84.6 & 90.7 & 70.3\\
     \rowcolor{vvlightgray}
     MIC \citep{mic}               & 82.6 & 89.1 & 68.4\\
     \rowcolor{vvlightgray}
     PADS \citep{roth2020pads}     & 83.5 & 89.7 & 68.8\\
     \hline
     Multisimilarity+\textit{SMSD}   & 86.3 $\pm$ 0.1 & 91.8 $\pm$ 0.3 & 72.0 $\pm$ 0.3\\
     Margin+\textit{SMSD}    & 86.0 $\pm$ 0.2 & 91.8 $\pm$ 0.2 & 72.2 $\pm$ 0.2 \\
     R-Margin+\textit{SMSD}  & \textbf{87.6} $\pm$ \textbf{0.2} & \textbf{92.7} $\pm$ \textbf{0.2} & \textbf{72.3} $\pm$ \textbf{0.2}\\
     \midrule
     \hline
     \multicolumn{4}{>{\columncolor[gray]{.8}}l}{\textbf{ResNet50-512}} \\
     \hline
     \rowcolor{vvlightgray}
     EPSHN \citep{epshn}                     & 82.7 & 89.3 &  -   \\
     \rowcolor{vvlightgray}
     NormSoft \citep{zhai2018classification} & 84.2 & 90.4 &  - \\     
     \rowcolor{vvlightgray}
     DiVA \citep{milbich2020diva}            & 87.6 & 92.9 & 72.2\\
     \hline
     Multisimilarity+\textit{SMSD}    & 89.1 $\pm$ 0.2 & 93.8 $\pm$ 0.2 & 74.0 $\pm$ 0.2\\
     Margin+\textit{SMSD}     & - $\pm$ - & - $\pm$ - & - $\pm$ - \\
     R-Margin+\textit{SMSD}   & 89.5 $\pm$ 0.2 & 93.8 $\pm$ 0.3 & 72.9 $\pm$ 0.3 \\
     % \red{N} DiVA+\textit{SMSD}   & - & - & - \\
     \midrule
     \hline
     \multicolumn{4}{>{\columncolor[gray]{.8}}l}{\textbf{Inception-BN-512}} \\
     \hline
    %  \rowcolor{vvlightgray}
    %  HORDE$^+$         & 83.9 & 90.3 & - \\
     \rowcolor{vvlightgray}
     DiVA \citep{milbich2020diva}   & 84.1 & 90.7 & 68.7\\
     \hline
     Multisimilarity+\textit{SMSD}   & 83.6 $\pm$ 0.3 & 90.3 $\pm$ 0.2 & 69.8 $\pm$ 0.3\\
     Margin+\textit{SMSD}            & 84.1 $\pm$ 0.2 & 90.6 $\pm$ 0.2 & 69.8 $\pm$ 0.2 \\
     R-Margin+\textit{SMSD}          & 83.8 $\pm$ 0.3 & 90.3 $\pm$ 0.2 & 69.4 $\pm$ 0.2\\
     \hline
     \rowcolor{vvlightgray}
     Softtriple$^*$ \citep{softriple} & 84.5 & 90.7 & 70.1\\
     \rowcolor{vvlightgray}
     Multisimilarity$^*$ \citep{multisimilarity} & 84.1 & 90.4 & -   \\
     \hline
     Multisimilarity$^*$+\textit{SMSD}   & 86.3 $\pm$ 0.2 & 92.2 $\pm$ 0.2 & 72.0 $\pm$ 0.3 \\
     Margin$^*$+\textit{SMSD}            & 87.1 $\pm$ 0.2 & 92.4 $\pm$ 0.1 & 72.2 $\pm$ 0.2 \\
     R-Margin$^*$+\textit{SMSD}          & 86.6 $\pm$ 0.3 & 92.1 $\pm$ 0.3 & 70.9 $\pm$ 0.2\\
     \hline
     \rowcolor{vvlightgray}
     ProxyAnchor$^{*\dagger}$ \citep{kim2020proxy}  & 86.1 & 91.7 & - \\
     \hline
     Multisimilarity$^{*\dagger}$+\textit{SMSD}      & 87.8 $\pm$ 0.2 & 93.1 $\pm$ 0.2 & 73.3 $\pm$ 0.3 \\
     Margin$^{*\dagger}$+\textit{SMSD}               & 87.6 $\pm$ 0.2 & 92.5 $\pm$ 0.2 & 72.6 $\pm$ 0.3 \\
     ProxyAnchor$^{*\dagger}$+\textit{SMSD}          & 87.2 $\pm$ 0.3 & 92.6 $\pm$ 0.2 & 70.5 $\pm$ 0.4\\
     % DiVA+\textit{SMSD}                            & - & - & -\\
     \bottomrule
\end{tabular}}

\vspace{5pt}

\resizebox{\textwidth}{!}{
 \begin{tabular}{l||c|c|c}
     \toprule
     Benchmark $\rightarrow$ & \multicolumn{3}{c}{SOP \citep{lifted}} \\
     \midrule
     Approach $\downarrow$ & R@1 & R@10 & NMI \\
     \midrule
     \hline
     \multicolumn{4}{>{\columncolor[gray]{.8}}l}{\textbf{ResNet50-128}} \\
     \hline
     \rowcolor{vvlightgray}
     Div\&Conq \citep{Sanakoyeu_2019_CVPR} & 75.9 & 88.4 & 90.2\\
     \rowcolor{vvlightgray}
     MIC \citep{mic}                  & 77.2 & 89.4 & 90.0\\
     \rowcolor{vvlightgray}
     PADS \citep{roth2020pads}        & 76.5 & 89.0 & 89.9\\
     \hline
     Multisimilarity+\textit{SMSD}     & 79.0 $\pm$ 0.2 & 90.2 $\pm$ 0.1 & 90.6 $\pm$ 0.1\\
     Margin+\textit{SMSD}              & 80.2 $\pm$ 0.2 & 91.5 $\pm$ 0.1 & 90.9 $\pm$ 0.1\\
     R-Margin+\textit{SMSD}            & 79.2 $\pm$ 0.2 & 90.3 $\pm$ 0.1 & 90.8 $\pm$ 0.1\\
     \midrule
     \hline
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
     \multicolumn{4}{>{\columncolor[gray]{.8}}l}{\textbf{ResNet50-512}} \\
     \hline
     \rowcolor{vvlightgray}
     EPSHN \citep{epshn}                     & 78.3 & 90.7 &  -   \\
     \rowcolor{vvlightgray}
     NormSoft \citep{zhai2018classification} & 78.2 & 90.6 &  -   \\          
     \rowcolor{vvlightgray}
     DiVA \citep{milbich2020diva}            & 79.6 & 91.2 & 90.6 \\
     \hline
     Multisimilarity+\textit{SMSD}  & 80.8 $\pm$ 0.2 & 92.2 $\pm$ 0.2 & 90.5 $\pm$ 0.3\\
     Margin+\textit{SMSD}           & 81.0 $\pm$ 0.2 & 92.1 $\pm$ 0.2 & 91.1 $\pm$ 0.3\\
     R-Margin+\textit{SMSD}         & 80.0 $\pm$ 0.2 & 91.4 $\pm$ 0.2 & 90.8 $\pm$ 0.1\\
     % \red{N} DiVA+\textit{SMSD}   & - & - & -\\
     \bottomrule
\end{tabular}




 \begin{tabular}{l||c|c|c}
     \toprule
     Benchmark $\rightarrow$ & \multicolumn{3}{c}{SOP \citep{lifted}} \\
     \midrule
     Approach $\downarrow$ & R@1 & R@10 & NMI \\
     \midrule
     \hline
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
     \multicolumn{4}{>{\columncolor[gray]{.8}}l}{\textbf{Inception-BN-512}} \\
     \hline
    %  \rowcolor{vvlightgray}
    %  HORDE$^+$         & 80.1      & 91.3      & -     \\
     \rowcolor{vvlightgray}
     DiVA \citep{milbich2020diva}   & 78.1 & 90.6 & 90.4\\
     \hline
     Multisimilarity+\textit{SMSD}   & 78.5 $\pm$ 0.2 & 90.6 $\pm$ 0.2 & 90.6 $\pm$ 0.1\\
     Margin$^*$+\textit{SMSD}        & 78.4 $\pm$ 0.2 & - $\pm$ - & 90.4 $\pm$ 0.1\\
     R-Margin$^*$+\textit{SMSD}      & 78.1 $\pm$ 0.2 & - $\pm$ - & 90.3 $\pm$ 0.2 \\     
     \hline
     \rowcolor{vvlightgray}
     Softtriple$^*$ \citep{softriple} & 78.3 & 90.3 & 92.0\\
     \rowcolor{vvlightgray}
     Multisimilarity$^*$ \citep{multisimilarity}   & 78.2 & 90.5 & -     \\
     \hline
     Multisimilarity$^*$+\textit{SMSD}       & 78.9 $\pm$ 0.2 & - $\pm$ - & 90.6 $\pm$ 0.1\\
     Margin+\textit{SMSD}            & 79.1 $\pm$ 0.2 & - $\pm$ - & 90.4 $\pm$ 0.1\\
     R-Margin+\textit{SMSD}          & 78.5 $\pm$ 0.1 & - $\pm$ - & 90.0 $\pm$ 0.2\\
     \hline
     \rowcolor{vvlightgray}
     ProxyAnchor$^{*\dagger}$ \citep{kim2020proxy}   & 79.1 & 90.8 & -\\
     \hline
     Multisimilarity$^{*\dagger}$+\textit{SMSD} & - $\pm$ - & - $\pm$ - & - $\pm$ -\\
     Margin$^{*\dagger}$+\textit{SMSD}          & - $\pm$ - & - $\pm$ - & - $\pm$ -\\
     ProxyAnchor$^{*\dagger}$+\textit{SMSD}     & - $\pm$ - & - $\pm$ - & - $\pm$ -\\
     % DiVA+\textit{SMSD}                            & - & - & -\\
     \bottomrule
\end{tabular}}


\vspace{-5pt}
\label{tab:sota}
\end{table*}


